MVSS-Net: Multi-View Multi-Scale Supervised Networks for Image Manipulation Detection

As manipulating images by copy-move, splicing and/or inpainting may lead to misinterpretation of the visual content, detecting these sorts of manipulations is crucial for media forensics. Given the variety of possible attacks on the content, devising a generic method is nontrivial. Current deep learning based methods are promising when training and test data are well aligned, but perform poorly on independent tests. Moreover, due to the absence of authentic test images, their image-level detection specificity is in doubt. The key question is how to design and train a deep neural network capable of learning generalizable features sensitive to manipulations in novel data, whilst specific to prevent false alarms on the authentic. We propose multi-view feature learning to jointly exploit tampering boundary artifacts and the noise view of the input image. As both clues are meant to be semantic-agnostic, the learned features are thus generalizable. For effectively learning from authentic images, we train with multi-scale (pixel / edge / image) supervision. We term the new network MVSS-Net and its enhanced version MVSS-Net++. Experiments are conducted in both within-dataset and cross-dataset scenarios, showing that MVSS-Net++ performs the best, and exhibits better robustness against JPEG compression, Gaussian blur and screenshot based image re-capturing.

==> backup.tex <==


\add{BayarConv learns noise features from data adpatively, providing better universality and robustness than handcrafted methods (\eg SRM filter)\cite{bayarvhandcraf}. It is applied as follows:}
\begin{equation} \label{eq:constrain}
\left\{ {\begin{array}{*{20}{c}}
{{\omega_k}\left( {0,0} \right) =  - 1}\\
{\sum\limits_{i,j \ne 0} {{\omega_k}\left( {i,j} \right) = 1} }
\end{array}} \right.
\end{equation}
\add{where ${\omega_k}$ denotes the $k^{th}$ convolution kernel, and $(0, 0)$ is
the center element of ${\omega_k}$. During training, ${\omega_k}$ is first updated with the entire model and then performed constraints according to Eq. \ref{eq:constrain}. 
Such constrain over center pixel is designed to estimate a set of prediction error filters. It aims at suppressing the content of image and learning local structural relationship\cite{prediction_error_filters}.} 



==> exp-ablation-hybridinfer.tex <==
\textbf{Influence of Hybrid Inference}. 
\add{
With hybrid inference strategy, \modelplus(HY)~achieves higher overall performance compared with \modelplus(HO), the holistic version.
We further elaborate their pixel-level F1 in different proportion of tampered area, see in Table \ref{table:tiny}.
Images with tiny manipulation area (size percentage less than 1\%) take up over half of manipulated part of DEFACTO-12k. 
From the left to the right, Table \ref{table:tiny} shows a common trend that the smaller the manipulated region is, the more difficult it is to be localized.
From the top to the bottom, a clear performance improvement can be observed with hybrid inference strategy. While \modelplus(HO)~improves performances on all areas of manipulations indiscriminately, hybrid inference strategy distinctly aims at tiny manipulations, see the top two lines and the bottom two lines of Table \ref{table:tiny} respectively. 
These results clearly demonstrate the superiority of hybrid inference strategy on tiny manipulations. Also Note that Table \ref{table:tiny} aims no comparison between SOTA works and our ablation models, as they are trained on different dataset. 
For a fair comparison one may refer to Section \ref{ssec:eval-sota}.} 
\input{table/table-patch}

==> table/table-backup.tex <==
\begin{table*}[htbp]
\caption{\textbf{Ablation study of \model}. Training: DEF-84k. Test: DEF-12k. F1, Sensitivity (\textit{Sen.}) and Specificity (\textit{Spe.}) scores are in percentage. Best number per column is highlighted in \textbf{bold}. The steadily improved performance justifies the necessity of the individual components used in \model~(Setup \#7) and \modelplus~(Setup \#9).}
% \renewcommand{\arraystretch}{1.05}
\begin{center}
\renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{1.5mm}
\footnotesize
\scalebox{1.05}{

%\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|r}
\begin{tabular}{l|cc|cccc|cccc|c}
\toprule
\multirow{2}{*}{\textbf{Setup}} &
  \multicolumn{2}{c|}{\textbf{Component}} &
  \multicolumn{4}{c|}{\textbf{Pixel-level manipulation detection (F1)}} &
  \multicolumn{4}{c|}{\textbf{Image-level manipulation detection}} &
  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Com-F1}}} \\ \cline{2-11}
 &
%   \textit{$\mathcal{G}_{clf}$} &
  \textit{ESB} &
  \textit{NSB} &
  \textit{cpmv.} &
  \textit{spli.} &
  \textit{inpa.} &
  \textit{MEAN} &
  \textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} &
  \multicolumn{1}{c}{} \\ \midrule
\multicolumn{12}{l}{\emph{Conference version}\cite{iccv21-mvssnet}, with GMP as $\mathcal{G}_{clf}$ } \\ 
%\midrule
~0:~Seg   & -                   & - & 45.3 & 72.2 & 46.3 & 54.6 & 0.840 & 82.7 & 62.0 & 70.9 & 61.7 \\ \hline
~1:~Seg+Clf  & -             & - & 34.1 & 67.3 & 37.6 & 46.3 & 0.858 & 76.8 & 77.8 & 77.3 & 57.9 \\ \hline
~2:~Seg+Clf+Noise   & -           & + & 39.3 & 70.6 & 42.6 & 50.8 & 0.871 & 76.3 & 82.1 & 79.1 & 61.9 \\ \hline
~3:~Seg+Clf+Edge   & +           & - & 40.5 & 71.5 & 43.5 & 51.8 & 0.870 & 77.3 & 81.1 & 79.2 & 62.6 \\ \hline
~4:~Seg+Clf+Edge/s  & w/o sobel & - & 38.2 & 71.0 & 42.2 & 50.5 & 0.869 & 79.2 & 78.9 & 79.0 & 61.6 \\ \hline
~5:~Seg+Clf+GSR  & GSR-Net     & - & 36.3 & 71.4 & 42.1 & 49.9 & 0.864 & 81.3 & 77.9 & 79.6 & 61.3 \\ \hline

~6:~Ensemble(\#2, \#3)  & + & + & 38.4 & 70.8 & 43.7 & 51.0 & 0.878 & 73.1 & 87.6 & 79.7 & 62.2 \\ \hline


~7: Seg+Clf+Noise+Edge  & + & + & 44.6 & 71.4 & 45.5 & 53.8 & 0.886 & 79.7 & 80.2 & \incolor{79.9} & 64.3 \\ \hline
\multicolumn{12}{l}{\emph{Journal extension, built on top of Setup \#7}} \\ 
%\midrule
% ~8:~\add{\model(P)} & GMP & + & + & 46.7 & 72.9 & 47.3 & 55.6 & 88.9 & 83.4 & 76.6 & 79.8 & 65.6 \\ \hline
~8: GeM as $\mathcal{G}_{clf}$  & + & + & 48.0  & 73.5 & 47.0 & 56.2 & 0.871 & 63.1 & 93.0 & 75.2 & 64.3 \\ \hline
  
~9: ConvGeM as $\mathcal{G}_{clf}$  & + & + & 48.3 & 72.8 & 49.0 & \incolor{56.7} & 0.879 & 74.8 & 85.7 & 79.8 & \incolor{66.3} \\ %\hline

%10: ConvGeM + HybridInfer (ss)  & + & + & 48.3 & 73.0 & 49.7 & 57.0 & 0.875 & 77.8 & 83.8 & 80.7 & 66.8 \\ \hline

%11: ConvGeM + HybridInfer (ms)  & + & + & \textbf{49.6} & \textbf{73.2} & \textbf{50.4} & \textbf{57.8} & 0.872 & 79.2 & 82.4 & \textbf{80.8} & \textbf{67.4} \\
\bottomrule
\end{tabular}%
}


\end{center}

\label{table:ablation}
\end{table*}

\begin{table*}[htbp]
\caption{\textbf{Performance of different models for pixel-level manipulation detection}. Performance metric: F1 [\%]. Best result per test set is highlighted in bold font. All models are trained on CASIAv2, except for those marked with star (*), the training data of which contains either private (ManTra-Net, SPAN, CAT-Net and HP-FCN) or published but no longer publicly accessible data (H-LSTM).} %All the models are trained on CASIAv2, except for ManTra-Net and HP-FCN.}
\renewcommand{\arraystretch}{1.2}
\begin{center}
\footnotesize
% \small
\setlength{\tabcolsep}{0.75mm}

%\resizebox{\textwidth}{!}{%
\scalebox{1}{
\begin{tabular}{l|ccccccc|ccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{7}{c|}{\textbf{Optimal threshold per model \& testset}} & \multicolumn{7}{c}{\textbf{Fixed threshold (0.5)}}  \\
\cline{2-15}
& \textit{NIST} & \textit{Columbia} & \textit{CASIAv1+}  & \textit{COVER}  & \textit{DEF-12k}  & \textit{IMD} & \textit{MEAN} & \textit{NIST} & \textit{Columbia} & \textit{CASIAv1+} & \textit{COVER}    & \textit{DEF-12k}    & \textit{IMD} & \textit{MEAN}  \\ \hline
MFCN, VCIR17\cite{2017MFCN}                   
& 42.2    & 61.2       & 54.1      & n.a.     & n.a.      & n.a.    & n.a.  & n.a.     & n.a.    & n.a.  & n.a.    & n.a. & n.a. &n.a.  \\
RGB-N, CVPR18\cite{2018rgbn}                  
& n.a.     & n.a.        & 40.8      & 37.9    & n.a.      & n.a.    & n.a.  & n.a.     & n.a.    & n.a.  & n.a.    & n.a. & n.a. & n.a.   \\
  
H-LSTM*, TIP19\cite{H-LSTM}
& 46.6  & 	14.2 &	20.9 &	21.3 &	12.5 &	31.0 & 24.4 & \incolor{35.4} &	13.0 &	15.4 &	16.3 	& ~~5.9 & 19.5 & 17.6 \\
HP-FCN*, ICCV19\cite{HPFCN}
& 36.0 &	47.1 &	21.4	& 19.9 &	13.6 & 16.9 & 25.8 & 12.1 &	~~6.7	& 15.4 &	~~0.3	& ~~5.5 & 11.2 & ~~8.5\\
ManTra-Net*, CVPR19\cite{mantranet}              
& 45.5    & 70.9       & 69.2      & 77.2    & \incolor{61.8}     & 70.5 &65.9  & ~~0.0 & 36.4    & 15.5   & 28.6 & \incolor{15.5}   & 18.7 & 19.1 \\

CR-CNN, ICME20\cite{2020Constrained}
& 42.8    & 70.4       & 66.2      & 47.0    & 34.0  &60.0   & 53.4   & 23.8 & 43.6    & 40.5   & 29.1 & 13.2   & 26.2  &29.4\\
GSR-Net, AAAI20\cite{2020GSR}                 
& 45.6    & 62.2       & 57.4      & 48.9    & 37.9     & 68.7  &53.4 & 28.3 & 61.3    & 38.7   & 28.5 & ~~5.1   & 24.3 &31.0\\
SPAN*, ECCV20\cite{2020SPAN} 
& 68.3 &	77.4 & 	68.8 &	71.8 &	57.1 &	69.6 & 68.8 & 22.1 &	48.7 & 	18.4 &	17.2 &	~~4.8 &	17.0&21.4\\
CAT-Net*, WACV20\cite{2021CAT} 
& 59.9 &	\incolor{77.6} &	57.3 &	48.5 &	44.1 &	51.7 & 56.5 & 17.9 &	55.5 &	13.6 & 	12.9 &	~~4.6 &	~~5.4 & 18.3 \\
\midrule
% \hline
% Res50-FCN16                 
% & 0.316    & 0.504       & 0.558      & 0.335    & 0.184     & 0.379   & 0.186 & 0.226    & 0.435   & 0.181 & 0.122   & 0.230 \\
% Res50-FCN16(DL)                 & 0.278    & 0.483       & 0.431      & 0.309    & 0.182     & 0.334   & 0.152 & 0.129    & 0.333   & 0.161 & 0.087   & 0.172 \\
%FCN                 & 0.507    & 0.586       & 0.742      & 0.573    & 0.401     & 0.562   & 0.167 & 0.223    & 0.441   & 0.199 & 0.130   & 0.232 \\
\multicolumn{15}{l}{\emph{This paper:}}\\
FCN & 50.7 &	58.6 &	74.2 &	57.3 &	40.1 &	64.5 & 57.6 & 16.7 &	22.3 &	44.1 &	19.9 &	13.0 &	21.0 & 22.8\\
\model,ICCV20\cite{iccv21-mvssnet} & 50.7    & 70.3       & 75.3      &  82.4    & 57.2     &  75.7  & 68.6  & 29.2 & 63.8    & 45.2   & 45.3 & 13.7   & 26.0 & 37.2 \\ 
\modelplus
& \incolor{73.7} & 73.1 &	\incolor{77.1} &	\incolor{83.2} &	55.6 &	\incolor{76.2} & \incolor{73.2} & 30.4 &	\incolor{66.0} &	\incolor{51.3} &	\incolor{48.2} & 	~~9.5 &	\incolor{27.0} &\incolor{38.7}\\

%\add{\modelplus(HY,ss)} &	60.3 &	73.9 &	\incolor{\textbf{78.8}} &	\incolor{\textbf{84.3}} &	55.5 &	68.7 	& 29.0 &	66.2 & 	52.0 &	48.8 &	9.8 &	26.8 \\
%\add{\modelplus(HY,ms)}	&	60.9 &	\incolor{\textbf{82.4}} &	77.6 &	74.1 & 55.7	&	67.4 &		29.3 &	\incolor{\textbf{66.3}} &	\incolor{\textbf{52.3}} &	\incolor{\textbf{49.1}} &	10.4 &	\incolor{\textbf{27.8}}\\
\bottomrule
\end{tabular}
}
\end{center}

\label{table:pix-f1}
%}
\end{table*}


\begin{table*}[htpb]
\caption{\textbf{Performance of image-level manipulation detection}. The NIST16 testset, which has no authentic images, is excluded. The default decision threshold of $0.5$ is used for all models.}
\renewcommand{\arraystretch}{1.25}
\begin{center}
%\small
\footnotesize
\setlength{\tabcolsep}{1.1mm}
%\resizebox{\textwidth}{!}{%
\scalebox{1}{
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} &
  \multicolumn{4}{c|}{\textbf{Columbia}} &
  \multicolumn{4}{c|}{\textbf{CASIAv1+}} &
  \multicolumn{4}{c|}{\textbf{COVER}} &
  \multicolumn{4}{c|}{\textbf{DEF-12k}} &
  \multicolumn{4}{c}{\textbf{\add{IMD}}}\\ \cline{2-21} 
\multicolumn{1}{c|}{} &
  \textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} &
  \textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} &
  \textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} &
\textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} &
  \textit{AUC} &
  \textit{Sen.} &
  \textit{Spe.} &
  \textit{F1} \\ \midrule
H-LSTM &
0.506 & 100.0 & 1.1 & 2.2 & 0.498 & 99.7 & 0.0 & 0.0 & 0.500 & 100.0 &	0.0 & 0.0 & 0.499 & 99.9 & 0.1 &  0.1 & 0.501 & 100.0 & 0.0 & 0.0 \\  
ManrTra-Net&
0.701 &	100.0 &	0.0 & 0.0 &	0.500 &	100.0 &	0.0 &	0.0 &	0.500 &	100.0 &	0.0 &	0.0 &	0.543 &	100.0 &	0.0 & 0.0 &	0.500 &	100.0 &	0.0 &	0.0 \\
C-RCNN &
0.783 &	96.1 &	24.6 &	39.2 &	0.719 &	93.0 &	13.9 &	24.2 &	0.566 &	96.7 &	7.0 &	13.1 &	0.567 &	77.4 &	26.7 &	39.7 &	0.615 &	92.9 &	12.3 &	21.8 \\
GSRNet &
0.502 &	100.0 &	1.1 &	2.2 &	0.500 &	99.4 &	0.0 &	0.0 &	0.515 &	100.0 &	0.0 &	0.0 &	0.456 &	91.4 &	0.1 &	0.2 &	0.500 &	100.0 &	0.0 &	0.0 \\

\add{SPAN} &
0.500 & 100.0 & 0.0 & 0.0 & 0.500 & 100.0 & 0.0 & 0.0 & 0.500 & 100.0 &	0.0 & 0.0 & 0.500 & 100.0 & 0.0 & 0.0 & 0.500 & 100.0 & 0.0 & 0.0 \\
\add{CAT-Net} &
0.971 & 87.2 & 96.2 & 91.5 & 0.647 & 23.9 & 92.1 & 38.0 & 0.557 & 28.0 &	80.0 & 41.5 & 0.543 & 34.2 & 72.5 & 46.4 & 0.586 & 27.5 & 81.6 & 41.1 \\\midrule
%\multicolumn{21}{l}{\emph{This paper:}}\\
FCN &
0.762 &	95.0 &	32.2 &	48.1 &	0.770 &	72.8 &	64.3 &	68.3 &	0.541 &	90.0 &	10.0 &	18.0 &	0.551 &	71.1 &	33.8 &	45.8 &	0.626 &	86.3 &	23.4 & 36.9 \\
\model &
0.980 & 66.9 & 100.0 & 80.2 & 0.937 & 61.5 & 98.8 & \incolor{75.8} & 0.731 & 94.0 &	14.0 & 24.4 & 0.573 & 81.7 & 26.8 & 40.4 & 0.656 & 91.5 & 22.0 & 35.4 \\
\add{\modelplus}&
0.984 & 96.7 & 89.6 & \incolor{93.0} & 0.862 & 53.6 & 98.4 & 69.4 & 0.726 & 69.0 &	68.0 & \incolor{68.5} & 0.531 & 37.3 &	66.6 &	\incolor{47.8}  & 0.645 & 59.5 & 63.5 & \incolor{61.4} \\ 
% \add{\modelplus(HY,ss)}	&	
% 0.986 &	98.9 &	81.4 &	89.3 &	0.821 &	63.8 &	89.1 &	74.4 &	0.729 &	72.0 &	64.0 &	67.8 &	0.530 &	37.3 &	67.2 &	47.9 & 0.657	&	79.4 &	40.8 &	53.9 \\
% \add{\modelplus(HY,ms)}&	
% 0.985 &	98.9 &	74.9 &	85.2 &	0.808 &	64.5 &	87.8 &	74.3 &	0.730 &	73.0 &	62.0 &	67.1 &	0.530 &	41.1 &	62.0 &	\textbf{49.4} &	0.638 &	84.5 &	24.6 &	38.2 \\\bottomrule

% ManrTra-Net & 0.701 & 1.000 & 0.000 & 0.000 & 0.500 & 1.000 & 0.000 & 0.000 & 0.491 & 1.000 & 0.000 & 0.000 & 0.543 & 1.000 & 0.000 & 0.000 & 0.500 & 1.000 & 0.000 & 0.000 \\

% CR-CNN    & 0.783 & 0.961 & 0.246 & 0.392 & 0.719 & 0.930 & 0.139 & 0.242 & 0.566 & 0.967 & 0.070 & 0.131 & 0.567 & 0.774 & 0.267 & 0.397 & 0.615 & 0.929 & 0.123 & 0.218\\
% GSR-Net     & 0.502 & 1.000 & 0.011 & 0.022 & 0.500 & 0.994 & 0.000 & 0.022 & 0.515 & 1.000 & 0.000 & 0.000 & 0.456 & 0.914 & 0.001 & 0.002 & 0.500 & 1.000 & 0.000 & 0.000 \\\midrule
% %FCN     & 0.762 & 0.950 & 0.322 & 0.481 & 0.796 & 0.717 & 0.844 & \textbf{0.775} & 0.541 & 0.900 & 0.100 & 0.180 & 0.551 & 0.711 & 0.338 & \textbf{0.458} \\
% \model   & \textbf{0.980} & 0.669 & 1.000 & \textbf{0.802} & \textbf{0.937} & 0.615 & 0.988 & 0.758 & \textbf{0.731} & 0.940 & 0.140  & \textbf{0.244} & \textbf{0.573} & 0.817 & 0.268 & 0.404 & 0.656 & 0.915 & 0.220 & 0.354 \\ 
\bottomrule
\end{tabular}%
}
\end{center}

\label{table:perf-img}
\end{table*}



==> table/table-patch.tex <==
\begin{table}[htbp]
\caption{\textbf{Pixel-level manipulation detection results of DEFACTO-12k in various manipulated area sizes.} The gap within each row shows the difficulty of detecting tiny manipulations, and the comparison within ablation models verifies the effectiveness of patch-inference strategy.}
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{0.8mm}
\scalebox{0.94}{
\begin{tabular}{llllll}
\toprule
% \multirow{3}{*}{Method} & \multicolumn{5}{c}{Proportion of Manipulated Area}            \\ \cline{2-6} 
\add{Size percentage}   & (0,0.005] & (0.005,0.01] & (0.01,0.05] & (0.05,0.1] & (0.1,1)  \\ %\cmidrule(lr){2-2} & \cmidrule(lr){3-3} &\cmidrule(lr){4-4} & \cmidrule(lr){5-5} & \cmidrule(lr){6-6} 
\add{Number percentage}            & 36.37\%          & 15.53\%    & 33.07\%   & 7.95\%   & 7.08\% \\ \midrule
\multicolumn{1}{l}{\textit{{SOTA works}}}  & \multicolumn{5}{l}{}                      \\ 
 \specialrule{0em}{2pt}{2pt}
H-LSTM	&0.015 				&0.041& 	0.098& 	0.114& 	0.088 \\
ManTra-Net&	0.055& 				0.138& 	0.245& 	0.281& 	0.406 \\
C-RCNN &	0.022& 				0.093& 	0.203& 	0.259& 	0.363\\ 
GSRNet&	0.012& 				0.024& 	0.082& 	0.104& 	0.119\\ 
SPAN&	0.011& 				0.025& 	0.073& 	0.093& 	0.114\\ 
CAT-Net&	0.016& 				0.034& 	0.057& 	0.099& 	0.116\\ \midrule
\multicolumn{5}{l}{\textit{{Ablation models trained on DEFACTO-84k	}}}  & \multicolumn{1}{l}{}\\ 
 \specialrule{0em}{2pt}{2pt}
							
\model               & 0.288            & 0.549      & 0.704     & 0.802    & 0.811  \\
\modelplus(HO)            & 0.303            & 0.568      & 0.736     & 0.825    & \textbf{0.840}  \\
\modelplus(HY,ss)&	0.308& 				0.582 &	0.741& 	0.820& 	0.825\\ 
\modelplus(HY,ms)           & \textbf{0.310~$\uparrow$}            & \textbf{0.592~$\uparrow$}      & \textbf{0.749~$\uparrow$}     & \textbf{0.831~$\uparrow$}    & 0.836~$\downarrow$  \\ \bottomrule
\end{tabular}
}
\label{table:tiny}
\end{table}


